CoDeR: Local Constraint-Compatible Retrieval Beyond Semantic Similarity

Information retrieval systems have long treated semantic similarity as a proxy for relevance. For constraint-sensitive queries, this proxy can fail when a document is topically close to the query but supports the opposite constraint direction, such as satisfying an attribute that should be excluded or affirming a relation that should be negated. We study this failure as constraint-violating evidence exposure and propose CoDeR, a local constraint-compatible dense retrieval method that separates topical relevance from constraint compatibility. CoDeR keeps a standard topical encoder for candidate coverage and adds a compatibility scorer, implemented as a bi-encoder, trained with lexical-polarity supervision over contrastive satisfying and violating evidences. The compatibility signal can be used to rescore topical candidates or to retrieve an auxiliary compatibility-oriented candidate set, producing a ranked document list without external Large Language Model~(LLM) calls at inference time. We evaluate CoDeR on controlled diagnostics and public negative-constraint retrieval benchmarks. Across three controlled diagnostic sets targeting antonymy, negation, and exclusion, CoDeR reduces V@2 by 20.59, 23.53, and 5.77 points relative to the strongest non-CoDeR baselines, and improves FVR by pushing the first violating document deeper in the ranking.

==> sec-xuebin-experiment.tex <==
\section{Experiments}
\label{sec:experiments}

This section evaluates whether CoDeR improves constraint-compatible retrieval without discarding the ordinary topical retrieval capability required by standard RAG pipelines. We organize the experiments around four questions: (i) whether CoDeR preserves retrieval quality on general BEIR benchmarks, (ii) whether it reduces topically relevant but constraint-violating evidence on diagnostic constraint-aware datasets, (iii) whether the same behavior transfers to previously published benchmarks, and (iv) whether the retrieval-side design improves efficiency relative to LLM-dependent baselines.

\subsection{Experimental Setup}
\label{subsec:experimental-setup}

\paragraph{Implementation and environment.}
All experiments are conducted on two GPU servers. The first server is equipped with an Intel(R) Xeon(R) Gold 6226R CPU @ 2.90GHz, 64 CPU cores, four Tesla V100S-PCIE-32GB GPUs, and 256GB RAM. The second server uses an AMD EPYC 7742 64-Core Processor, 32 CPU cores, three NVIDIA A100-PCIE-40GB GPUs, and 512GB RAM.

\paragraph{Datasets.}
We evaluate CoDeR on three groups of datasets. First, to test whether constraint-aware retrieval harms ordinary topical retrieval, we use six BEIR-format benchmarks: SciFact, ArguAna, FiQA, NFCorpus, Cqadupstack-android, and SciDocs. The Cqadupstack-android subset is taken from the BEIR Cqadupstack collection, and the other BEIR-format datasets are obtained from the BEIR repository. Second, we construct three diagnostic test sets for antonym, negation, and exclusion constraints from SciFact, SciDocs, and NFCorpus, respectively. These datasets contain 307, 304, and 312 documents, and 103, 104, and 104 query instances. Third, we evaluate on published constraint-aware benchmarks, including NevIR, ExcluIR, and NegConstraint. NevIR is a negative-constraint retrieval benchmark released at \url{https://github.com/orionw/NevIR.git}. ExcluIR is an exclusion-oriented retrieval benchmark released at \url{https://github.com/zwh-sdu/ExcluIR.git}. NegConstraint was introduced by NS-IR for negative-constraint retrieval. It was originally constructed from Wikipedia documents with human-annotated positive and negative documents under several negative-constraint formulations. Since the released version is incomplete and does not include the full category labels described in the original paper, we evaluate on the available released data only.

\paragraph{Construction of diagnostic constraint-aware datasets.}
The self-constructed datasets are designed to isolate the failure mode described by Eq.~\ref{eq:constraint_compatible_objective}: a document can be highly topical while supporting the opposite constraint direction. For the antonym dataset, we first select candidate documents from the SciFact corpus according to the number of sentences and tokens. Each selected document is semantically segmented into multiple sub-documents. We then ask GPT-5.5 to choose one sub-document and one keyword appearing in it that has an antonym, and to synthesize a query that contains the keyword while remaining topically relevant to the source document. Next, we create a paired document by replacing only that keyword with its antonym, while keeping the resulting text fluent and semantically consistent with the surrounding context. We also generate a paired query by replacing the keyword in the original query with its antonym. For each query pair, the topical relevant set is shared by both queries and includes all sub-documents extracted from the source document as well as the antonym-replaced document. The constraint-satisfying and constraint-violating documents are swapped between the two queries. We assign graded relevance scores of 2.0 to constraint-satisfying documents, 1.0 to neutral topical documents, and 0.0 to constraint-violating documents.

The negation and exclusion datasets follow the same construction protocol, but use different lexical operators. In the negation setting, the target word is replaced by a negated form such as ``not'' or ``no''. In the exclusion setting, the target word is replaced by an exclusion cue such as ``excluding'' or ``without''. This construction yields paired cases in which topical overlap is deliberately preserved while the constraint direction changes.

\paragraph{Compared methods.}
We compare CoDeR with sparse retrieval, dense retrieval, and LLM-dependent retrieval baselines. BM25 represents lexical sparse retrieval. BGE and Contriever represent dense embedding retrievers. HyDE generates hypothetical documents for retrieval and uses them as expanded retrieval queries. NS-IR applies LLM-based query-side optimization for negative constraints. DEO is an LLM-dependent method for negation- and exclusion-aware retrieval. For the strong LLM-dependent baselines, we follow their public implementations where available: HyDE at \url{https://github.com/texttron/hyde.git}, NS-IR at \url{https://github.com/xgl-git/NS-IR-main.git}, and DEO at \url{https://github.com/taegyeong-lee/DEO-negation-aware-retrieval.git}. CoDeR$_{\text{v1}}$ denotes the sequential integration policy that applies the constraint encoder after topical retrieval, while CoDeR$_{\text{v2}}$ denotes the union candidate integration policy that allows both the topical encoder and the constraint encoder to contribute candidates before normalized fusion and relative filtering.

\paragraph{Evaluation metrics.}
On standard BEIR datasets, we report nDCG@10 and MAP@10. On constraint-aware datasets, we report nDCG@10 together with the violation metrics defined in Eq.~\ref{eq:violation_at_k} and Eq.~\ref{eq:first_violating_rank}. V@$k$ is the percentage of queries for which at least one violating document appears within the top $k$ retrieved documents; lower values indicate safer retrieved context. FVR measures the first violating rank, where larger values indicate that violating evidence is pushed farther down the ranking. For NegConstraint, we follow the dataset convention and report Recall@5, nDCG@5, and MAP@10. We also report wall-clock inference time, API cost, and API token consumption for LLM-dependent methods and CoDeR variants.

\paragraph{Example query pairs.}
Table~\ref{tab:dataset_examples} shows one representative query pair from each diagnostic dataset together with its paired corpus snippets. The examples illustrate that the paired documents are intentionally close in topic and surface form, while differing in the direction of the expressed constraint.

\begin{table*}[t]
\centering
\small
\setlength{\tabcolsep}{6pt}
\renewcommand{\arraystretch}{1.20}
\begin{tabular}{p{0.14\textwidth} p{0.40\textwidth} p{0.40\textwidth}}
\hline
Dataset & Query pair & Paired corpus \\
\hline
\textbf{Antonym} & With \textbf{ \underline{appropriate} } validation, BRCA mutation-location findings may support cancer risk assessment. & With \textbf{ \underline{appropriate} } validation, mutation-location findings may support cancer risk assessment and prevention decision making for BRCA1 and BRCA2 mutation carriers. \\
& With \textbf{ \underline{inappropriate} } validation, BRCA mutation-location findings may support cancer risk assessment. & With \textbf{ \underline{inappropriate} } validation, mutation-location findings may support cancer risk assessment and prevention decision making for BRCA1 and BRCA2 mutation carriers. \\
\hline
\textbf{Negation} & HGAPSO demonstrates \textbf{ \underline{superiority} } over GA and PSO in recurrent network design problems. & The performance of HGAPSO is compared with both GA and PSO in recurrent network design problems, demonstrating \textbf{ \underline{superiority} }. \\
& HGAPSO demonstrates \textbf{ \underline{no superiority} } over GA and PSO in recurrent network design problems. & The performance of HGAPSO is compared with both GA and PSO in recurrent network design problems, demonstrating \textbf{ \underline{no superiority} }. \\
\hline
\textbf{Exclusion} & The two groups were compared for changes in semen parameters and \textbf{ \underline{total seminal plasma antioxidant capacity} }. & The effect of saffron was evaluated compared with placebo for the treatment of idiopathic male factor infertility. The two groups were compared for changes in semen parameters and \textbf{ \underline{total seminal plasma antioxidant capacity} }. \\
& The two groups were compared for changes in semen parameters, \textbf{ \underline{excluding} } total seminal plasma antioxidant capacity. & The effect of saffron was evaluated compared with placebo for the treatment of idiopathic male factor infertility. The two groups were compared for changes in semen parameters, \textbf{ \underline{excluding} } total seminal plasma antioxidant capacity. \\
\hline
\end{tabular}
\caption{Representative query pairs and paired corpus snippets from the three self-constructed test sets.}
\label{tab:dataset_examples}
\end{table*}


\subsection{Main Retrieval Results}
\label{subsec:experimental-results}
 
\paragraph{General BEIR datasets.}
Table~\ref{tab:beir} reports the performance of all compared methods on six BEIR benchmark datasets. We include nDCG@10 and MAP@10 as retrieval quality metrics. The best results in each column are highlighted in \textbf{bold}. These datasets do not specifically target constraint violations, so they test whether adding a compatibility signal damages ordinary topical retrieval quality.
 
\begin{table*}[h]
    \small
    \centering
    \resizebox{\textwidth}{!}{
    \begin{tabular}{l|cc|cc|cc|cc|cc|cc}
        \toprule
        \multirow{2.5}{*}{Methods}
        & \multicolumn{2}{c|}{SciFact}
        & \multicolumn{2}{c|}{ArguAna}
        & \multicolumn{2}{c|}{FiQA}
        & \multicolumn{2}{c|}{NFCorpus}
        & \multicolumn{2}{c|}{\makecell{CQA\\Android}}
        & \multicolumn{2}{c}{SciDocs} \\
        \cmidrule{2-3}\cmidrule{4-5}\cmidrule{6-7}\cmidrule{8-9}\cmidrule{10-11}\cmidrule{12-13}
        & nDCG & MAP & nDCG & MAP & nDCG & MAP & nDCG & MAP & nDCG & MAP & nDCG & MAP \\
        \midrule
        BM25 
        & 64.82 & 60.37 
        & 34.40 & 22.56 
        & 23.25 & 17.20 
        & 30.98 & 22.36 
        & 39.08 & 34.32 
        & 15.04 & 8.76 \\

        BGE 
        & 74.77 & 69.93 
        & 45.99 & 32.25 
        & 45.00 & 37.15 
        & \textbf{38.15} & \textbf{28.76}
        & \textbf{50.22} & \textbf{43.89}
        & \textbf{22.63} & \textbf{13.80} \\

        Contriever 
        & 55.04 & 49.43 
        & 33.55 & 21.90 
        & 12.41 & 8.81 
        & 27.12 & 18.62 
        & 30.37 & 25.56 
        & 10.97 & 5.85 \\

        HyDE 
        & 67.44 & 61.98 
        & 30.41 & 19.28 
        & 28.51 & 22.16 
        & 31.59 & 22.46 
        & 21.55 & 17.56 
        & 14.21 & 7.95 \\

        NS-IR 
        & 74.44 & 69.92 
        & 45.35 & 32.31 
        & 42.68 & 34.80 
        & 36.92 & 27.66 
        & 49.94 & 43.61 
        & 22.59 & 13.42 \\

        DEO 
        & 72.09 & 67.19 
        & \textbf{70.27} & \textbf{63.08}
        & 43.62 & 35.56 
        & 36.68 & 14.27 
        & 44.59 & 37.91 
        & 22.33 & 13.47 \\
        
        \midrule

        CoDeR$_{\text{v1}}$ 
        & 74.77 & 69.93 
        & 49.36 & 35.40 
        & \textbf{45.00} & \textbf{37.15} 
        & 37.24 & 28.00 
        & 48.02 & 42.15 
        & 21.42 & 12.86 \\

        CoDeR$_{\text{v2}}$ 
        & \textbf{74.91} & \textbf{70.17}
        & 48.78 & 35.00 
        & 44.51 & 36.80 
        & 36.36 & 27.12 
        & 48.17 & 42.22 
        & 21.60 & 12.96 \\

        \bottomrule
    \end{tabular}
    }
    \caption{Performance comparison on BEIR benchmark datasets. For each dataset, both nDCG and MAP are reported at @10. CQA Android refers to the Cqadupstack-android subset.}
    \label{tab:beir}
\end{table*}
 
Overall, CoDeR maintains competitive topical retrieval performance on ordinary BEIR datasets. On SciFact, CoDeR$_{\text{v2}}$ obtains the best nDCG@10 and MAP@10, slightly improving over BGE. On FiQA, CoDeR$_{\text{v1}}$ matches BGE, while CoDeR$_{\text{v2}}$ remains close. On NFCorpus, Cqadupstack-android, and SciDocs, BGE is strongest, but the CoDeR variants remain near the dense-retrieval baseline. The main exception is ArguAna, where DEO achieves substantially higher scores. These results indicate that introducing constraint compatibility does not collapse general-purpose retrieval quality, which is important because a RAG retriever must still preserve topical coverage when no explicit constraint conflict is present.

\paragraph{Diagnostic constraint-aware datasets.}
Table~\ref{tab:selfbuilt} reports results on our three self-constructed datasets covering Antonym, Negation, and Exclusion query types. We report nDCG@10, Violation Rate metrics (V@2, V@3, V@5, V@10), and FVR.
 
\begin{table*}[h]
    \small
    \centering
    \resizebox{\textwidth}{!}{
    \begin{tabular}{l|cccccc|cccccc|cccccc}
        \toprule
        \multirow{2.5}{*}{Methods}
        & \multicolumn{6}{c|}{Antonym}
        & \multicolumn{6}{c|}{Negation}
        & \multicolumn{6}{c}{Exclusion} \\
        \cmidrule{2-7}\cmidrule{8-13}\cmidrule{14-19}
        & nDCG & V@2 & V@3 & V@5 & V@10 & FVR
        & nDCG & V@2 & V@3 & V@5 & V@10 & FVR
        & nDCG & V@2 & V@3 & V@5 & V@10 & FVR \\
        \midrule
        BM25       
        & 78.43 & 90.20 & 98.04 & 100.00 & 100.00 & 2.11
        & 78.44 & 98.03 & 100.00 & 100.00 & 100.00 & 2.00
        & 73.24 & 76.47 & 87.25 & 97.06 & 100.00 & 2.26 \\
        
        BGE        
        & 83.92 & 81.37 & 92.16 & 99.02 & 100.00 & 2.30
        & 83.49 & 90.20 & 96.08 & 100.00 & 100.00 & 2.02
        & 77.48 & 69.61 & 82.35 & 88.24 & 95.10 & 2.93 \\
        
        Contriever 
        & 83.37 & 78.43 & 95.10 & 100.00 & 100.00 & 2.21
        & 83.83 & 83.33 & 92.16 & 99.02 & 100.00 & 2.25
        & 76.83 & 77.45 & 89.22 & 96.08 & 100.00 & 2.20 \\
        
        HyDE       
        & 82.09 & 82.35 & 92.16 & 100.00 & 100.00 & 2.08
        & 81.14 & 84.31 & 91.18 & 99.02 & 100.00 & 2.06
        & 76.73 & 66.67 & 83.33 & 96.08 & 99.02 & 2.48 \\
        
        NS-IR      
        & \textbf{86.16} & 75.49 & 92.16 & 99.02 & 100.00 & 2.34
        & \textbf{84.83} & 84.31 & 97.06 & 100.00 & 100.00 & 2.15
        & \textbf{77.96} & 68.63 & 81.37 & 92.16 & 99.02 & 2.72 \\
        
        DEO        
        & 82.65 & 73.53 & 85.29 & 98.04 & 100.00 & 2.42
        & 79.38 & 72.55 & 86.27 & 94.12 & 97.06 & 2.68
        & 76.21 & 53.85 & 71.15 & 79.81 & 88.46 & 3.76 \\
        
        \midrule
        
        CoDeR$_{\text{v1}}$ 
        & 82.70 & 59.80 & \textbf{76.47} & \textbf{91.18} & 99.02 & 2.95
        & 80.14 & 50.98 & 73.53 & \textbf{84.31} & 92.16 & \textbf{3.53}
        & 77.03 & 50.00 & \textbf{60.58} & \textbf{74.04} & 84.62 & 4.26 \\
        
        CoDeR$_{\text{v2}}$ 
        & 82.72 & \textbf{52.94} & \textbf{76.47} & 93.13 & \textbf{98.04} & \textbf{3.00}
        & 79.75 & \textbf{49.02} & \textbf{72.55} & 89.22 & \textbf{90.20} & 3.47
        & 76.23 & \textbf{48.08} & 61.54 & 75.96 & \textbf{81.73} & \textbf{4.37} \\
        
        \bottomrule
    \end{tabular}
    }
    \caption{Performance on self-constructed Antonym, Negation, and Exclusion datasets. nDCG is reported at @10. V@$k$ denotes the Violation Rate at rank $k$; FVR denotes the first violating rank.}
    \label{tab:selfbuilt}
\end{table*}
 
The diagnostic datasets expose a different behavior from standard BEIR evaluation. Methods with strong nDCG can still retrieve violating documents early because the violating documents are deliberately topical. CoDeR substantially reduces early violations across all three constraint types. For Antonym, CoDeR$_{\text{v2}}$ reduces V@2 from 81.37 for BGE and 75.49 for NS-IR to 52.94, while increasing FVR to 3.00. For Negation, CoDeR$_{\text{v2}}$ reaches the lowest V@2 and V@10, reducing V@2 to 49.02 compared with 90.20 for BGE and 84.31 for NS-IR. For Exclusion, CoDeR$_{\text{v2}}$ reduces V@2 to 48.08 and V@10 to 81.73, while achieving the highest FVR. These improvements come with a moderate nDCG trade-off because CoDeR suppresses some documents that are topically relevant but constraint-incompatible. This trade-off is expected under our objective: for constraint-sensitive RAG, the safer ranking is not necessarily the ranking with the highest topical score alone.

\paragraph{Published constraint-aware benchmarks.}
Table~\ref{tab:benchmarks} reports performance on NevIR and ExcluIR, two publicly released benchmarks for negative-constraint and exclusion-based retrieval. We report nDCG@10, V@$k$, and FVR. Table~\ref{tab:negconstraint} further reports results on NegConstraint, the negative-constraint benchmark introduced by NS-IR. Because the released NegConstraint data are incomplete and do not provide the full category labels described in the original paper, we report the available retrieval metrics on the released subset.
 
\begin{table*}[h]
    \small
    \centering
    \resizebox{\textwidth}{!}{
    \begin{tabular}{l|cccccc|cccccc}
        \toprule
        \multirow{2.5}{*}{Methods}
        & \multicolumn{6}{c|}{NevIR}
        & \multicolumn{6}{c}{ExcluIR} \\
        \cmidrule{2-7}\cmidrule{8-13}
        & nDCG & V@2 & V@3 & V@5 & V@10 & FVR
        & nDCG & V@2 & V@3 & V@5 & V@10 & FVR \\
        \midrule
        BM25       
        & 56.15 & 43.00 & 65.20 & 85.00 & 90.40 & 3.56
        & 80.61 & 90.20 & 93.90 & 96.60 & 97.70 & 1.94 \\
        
        BGE        
        & 60.69 & 36.80 & 60.30 & 85.60 & 90.30 & 3.70
        & 82.93 & 96.10 & 97.70 & 98.20 & 99.10 & 1.75 \\
        
        Contriever 
        & 57.50 & 42.10 & 64.40 & 84.20 & 88.50 & 3.69
        & 80.52 & 91.60 & 93.90 & 96.20 & 98.00 & 1.91 \\
        
        HyDE       
        & 57.79 & 41.30 & 63.40 & 86.10 & 90.00 & 3.58
        & 92.35 & 57.40 & 66.00 & 75.00 & 81.80 & 4.21 \\
        
        NS-IR      
        & 60.69 & 35.80 & 60.90 & 84.80 & 91.40 & 3.71
        & 84.17 & 95.60 & 97.10 & 98.10 & 98.70 & 1.79 \\
        
        DEO        
        & 59.19 & 31.10 & 56.50 & 81.90 & 88.60 & 4.02
        & \textbf{93.50} & 51.10 & 59.60 & 66.10 & 74.30 & 4.93 \\
        
        \midrule
        
        CoDeR$_{\text{v1}}$ 
        & \textbf{60.91} & \textbf{28.50} & \textbf{52.90} & 79.40 & 86.20 & 4.26
        & 92.99 & 47.70 & \textbf{56.60} & \textbf{64.40} & 73.70 & 5.06 \\
        
        CoDeR$_{\text{v2}}$ 
        & 59.62 & 30.20 & 53.20 & \textbf{78.80} & \textbf{86.00} & \textbf{4.28}
        & 92.78 & \textbf{45.00} & 57.20 & 65.30 & \textbf{65.70} & \textbf{5.33} \\
        
        \bottomrule
    \end{tabular}
    }
    \caption{Performance on published benchmark datasets NevIR and ExcluIR. nDCG is reported at @10. V@$k$ denotes the Violation Rate at rank $k$; FVR denotes the first violating rank.}
    \label{tab:benchmarks}
\end{table*}
 
The published benchmarks confirm that the violation-control behavior transfers beyond our diagnostic construction. On NevIR, CoDeR$_{\text{v1}}$ obtains the best nDCG@10 and the lowest V@2 and V@3, while CoDeR$_{\text{v2}}$ gives the lowest V@5 and V@10 and the highest FVR. On ExcluIR, DEO achieves the highest nDCG@10, but CoDeR$_{\text{v2}}$ produces the lowest V@2 and V@10 and the highest FVR. This again reveals a distinction between relevance-oriented ranking and constraint-safe context selection. Some methods can score highly in nDCG while still placing violating evidence near the top; CoDeR is designed to reduce this risk by explicitly modeling compatibility.

\begin{table}[h]
    \small
    \centering
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{l|ccc}
        \toprule
        \multicolumn{1}{c|}{Methods}
        & Recall@5
        & nDCG@5
        & MAP@10 \\
        \midrule
        NS-IR      & 95.96 & 76.64 & 70.05 \\
        \midrule
        CoDeR$_{\text{v1}}$ & 96.46 & 81.20 & 76.00 \\
        CoDeR$_{\text{v2}}$ & \textbf{96.97} & \textbf{81.61} & \textbf{76.38} \\
        \bottomrule
    \end{tabular}
    }
    \caption{Performance on the NegConstraint dataset. Recall@5, nDCG@5, and MAP@10 are reported.}
    \label{tab:negconstraint}
\end{table}
 
On NegConstraint, both CoDeR variants outperform NS-IR on all reported metrics. CoDeR$_{\text{v2}}$ obtains the best Recall@5, nDCG@5, and MAP@10, improving MAP@10 from 70.05 to 76.38. Although this evaluation is limited by the incomplete released version of NegConstraint, the improvement suggests that the compatibility encoder can provide useful retrieval-side supervision for negative-constraint queries beyond the paired lexical transformations used in our own benchmark construction.

\subsection{Efficiency Analysis}
\label{subsec:efficiency-analysis}

\paragraph{Efficiency comparison.}
Table~\ref{tab:efficiency} compares the computational efficiency of LLM-dependent baselines (HyDE, NS-IR, and DEO) with our CoDeR variants on the five constraint-aware datasets. Since CoDeR performs no LLM calls at inference time, it incurs zero API cost and zero token consumption on all datasets. In terms of wall-clock time, CoDeR is substantially faster than HyDE and NS-IR, especially on NevIR and ExcluIR, where it reduces inference time by three to four orders of magnitude.
 
\begin{table*}[h]
    \small
    \centering
    \resizebox{\textwidth}{!}{
    \begin{tabular}{l|ccc|ccc|ccc|ccc|ccc}
        \toprule
        \multirow{2.5}{*}{Methods}
        & \multicolumn{3}{c|}{Antonym}
        & \multicolumn{3}{c|}{Negation}
        & \multicolumn{3}{c|}{Exclusion}
        & \multicolumn{3}{c|}{NevIR}
        & \multicolumn{3}{c}{ExcluIR} \\
        \cmidrule{2-4}\cmidrule{5-7}\cmidrule{8-10}\cmidrule{11-13}\cmidrule{14-16}
        & Time & Cost & Token
        & Time & Cost & Token
        & Time & Cost & Token
        & Time & Cost & Token
        & Time & Cost & Token \\
        \midrule
        HyDE
        & 3,901 & \$1.22 & 146.3K
        & 3,223 & \$1.24 & 148.8K
        & 4,232 & \$1.00 & 124.1K
        & 56,204 & \$9.81 & 1,183.0K
        & 69,233 & \$13.85 & 1,668.9K \\
 
        NS-IR
        & 7,190 & \$0.85 & 128.8K
        & 6,979 & \$0.98 & 144.0K
        & 8,249 & \$1.27 & 177.9K
        & 61,621 & \$5.18 & 755.3K
        & 69,775 & \$10.65 & 1,501.5K \\
 
        DEO
        & 181 & \$0.18 & 50.5K
        & 187 & \$0.18 & 50.9K
        & 190 & \$0.19 & 51.9K
        & 16,516 & \$1.70 & 487.7K
        & 17,621 & \$2.03 & 531.4K \\
 
        \midrule
 
        CoDeR$_{\text{v1}}$
        & \textbf{6} & \textbf{0} & \textbf{0}
        & \textbf{6} & \textbf{0} & \textbf{0}
        & \textbf{7} & \textbf{0} & \textbf{0}
        & 131 & \textbf{0} & \textbf{0}
        & \textbf{67} & \textbf{0} & \textbf{0} \\
 
        CoDeR$_{\text{v2}}$
        & \textbf{6} & \textbf{0} & \textbf{0}
        & 7 & \textbf{0} & \textbf{0}
        & 8 & \textbf{0} & \textbf{0}
        & \textbf{66} & \textbf{0} & \textbf{0}
        & 89 & \textbf{0} & \textbf{0} \\
 
        \bottomrule
    \end{tabular}
    }
    \caption{Efficiency comparison on constraint-aware datasets. Time is reported in seconds, API cost is reported in US dollars, and API token count is reported in thousands (K). The best results in each column are highlighted in \textbf{bold}.}
    \label{tab:efficiency}
\end{table*}
 
The efficiency results highlight a key deployment advantage of retrieval-side compatibility scoring. HyDE, NS-IR, and DEO require external model calls and therefore incur both latency and API cost. CoDeR instead uses local encoder scoring after training. On the three self-constructed datasets, CoDeR finishes in single-digit seconds, while HyDE and NS-IR require thousands of seconds. On NevIR and ExcluIR, the gap is even larger: CoDeR completes evaluation in tens to hundreds of seconds, while HyDE and NS-IR require more than fifty thousand seconds. This makes CoDeR suitable for privacy-sensitive or cost-sensitive RAG systems where issuing additional LLM calls for every query is undesirable.

\subsection{Ablation Study}
\label{subsec:ablation-study}

Tables~\ref{tab:ablation_v1} and~\ref{tab:ablation_v2} reserve the ablation protocol for CoDeR$_{\text{v1}}$ and CoDeR$_{\text{v2}}$, respectively. The ablations evaluate two design questions: how the topical encoder affects the final ranking when the compatibility encoder is fixed, and how the compatibility encoder affects constraint safety when the topical encoder is fixed. Each variant is evaluated on SciFact and NFCorpus with nDCG@10 and MAP@10, and on the three self-constructed diagnostic datasets with nDCG@10, V@$k$, and FVR. The numerical entries are left open until the ablation runs are completed; therefore, we do not draw quantitative conclusions from these tables in the current draft.
 
\begin{table*}[h]
    \small
    \centering
    \resizebox{\textwidth}{!}{
    \begin{tabular}{ll|cc|cc|cccccc|cccccc|cccccc}
        \toprule
        \multirow{2.5}{*}{Encoder A} & \multirow{2.5}{*}{Encoder B}
        & \multicolumn{2}{c|}{SciFact} & \multicolumn{2}{c|}{NFCorpus}
        & \multicolumn{6}{c|}{Antonym} & \multicolumn{6}{c|}{Negation} & \multicolumn{6}{c}{Exclusion} \\
        \cmidrule{3-4}\cmidrule{5-6}\cmidrule{7-12}\cmidrule{13-18}\cmidrule{19-24}
        & & \makecell{nDCG} & \makecell{MAP}
          & \makecell{nDCG} & \makecell{MAP}
          & \makecell{nDCG} & V@2 & V@3 & V@5 & V@10 & FVR
          & \makecell{nDCG} & V@2 & V@3 & V@5 & V@10 & FVR
          & \makecell{nDCG} & V@2 & V@3 & V@5 & V@10 & FVR \\
        \midrule
        \multicolumn{24}{l}{\textit{Group 1: Fix Encoder B = CoDeR$_{\text{v1}}$, vary Encoder A}} \\
        \midrule
        BGE-large  & CoDeR$_{\text{v1}}$ & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
        BGE-base   & CoDeR$_{\text{v1}}$ & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
        BGE-small  & CoDeR$_{\text{v1}}$ & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
        \midrule
        \multicolumn{24}{l}{\textit{Group 2: Fix Encoder A = BGE-large, vary Encoder B}} \\
        \midrule
        BGE-large  & CoDeR$_{\text{v1}}$ & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
        BGE-large  & Contriever          & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
        BGE-large  & miniLM              & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
        \bottomrule
    \end{tabular}
    }
    \caption{Ablation study for CoDeR$_{\text{v1}}$. nDCG and MAP are reported at @10. Group~1 fixes Encoder~B as CoDeR$_{\text{v1}}$ and varies Encoder~A among BGE-large, BGE-base, and BGE-small. Group~2 fixes Encoder~A as BGE-large and varies Encoder~B among CoDeR$_{\text{v1}}$, Contriever, and miniLM.}
    \label{tab:ablation_v1}
\end{table*}
 
\begin{table*}[h]
    \small
    \centering
    \resizebox{\textwidth}{!}{
    \begin{tabular}{ll|cc|cc|cccccc|cccccc|cccccc}
        \toprule
        \multirow{2.5}{*}{Encoder A} & \multirow{2.5}{*}{Encoder B}
        & \multicolumn{2}{c|}{SciFact} & \multicolumn{2}{c|}{NFCorpus}
        & \multicolumn{6}{c|}{Antonym} & \multicolumn{6}{c|}{Negation} & \multicolumn{6}{c}{Exclusion} \\
        \cmidrule{3-4}\cmidrule{5-6}\cmidrule{7-12}\cmidrule{13-18}\cmidrule{19-24}
        & & \makecell{nDCG} & \makecell{MAP}
          & \makecell{nDCG} & \makecell{MAP}
          & \makecell{nDCG} & V@2 & V@3 & V@5 & V@10 & FVR
          & \makecell{nDCG} & V@2 & V@3 & V@5 & V@10 & FVR
          & \makecell{nDCG} & V@2 & V@3 & V@5 & V@10 & FVR \\
        \midrule
        \multicolumn{24}{l}{\textit{Group 1: Fix Encoder B = CoDeR$_{\text{v2}}$, vary Encoder A}} \\
        \midrule
        BGE-large  & CoDeR$_{\text{v2}}$ & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
        BGE-base   & CoDeR$_{\text{v2}}$ & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
        BGE-small  & CoDeR$_{\text{v2}}$ & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
        \midrule
        \multicolumn{24}{l}{\textit{Group 2: Fix Encoder A = BGE-large, vary Encoder B}} \\
        \midrule
        BGE-large  & CoDeR$_{\text{v2}}$ & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
        \rowcolor[rgb]{.9,.9,.9}
        BGE-large  & Contriever          & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
        BGE-large  & miniLM              & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
        \bottomrule
    \end{tabular}
    }
    \caption{Ablation study for CoDeR$_{\text{v2}}$. nDCG and MAP are reported at @10. Group~1 fixes Encoder~B as CoDeR$_{\text{v2}}$ and varies Encoder~A among BGE-large, BGE-base, and BGE-small. Group~2 fixes Encoder~A as BGE-large and varies Encoder~B among CoDeR$_{\text{v2}}$, Contriever, and miniLM.}
    \label{tab:ablation_v2}
\end{table*}

\subsection{Discussion and Analysis}
\label{subsec:discussion-analysis}

The experiments show that constraint-compatible retrieval should be evaluated with both topical relevance metrics and violation-aware diagnostics. Standard nDCG and MAP remain necessary because a constraint-aware retriever must still retrieve documents about the user's information need. However, these metrics alone do not distinguish a satisfying document from a topically similar document that supports the opposite constraint direction. The diagnostic datasets, NevIR, and ExcluIR make this distinction explicit through V@$k$ and FVR, while NegConstraint provides an additional published negative-constraint test case under its released evaluation format.

Across the constraint-aware evaluations, CoDeR consistently reduces early exposure to violating evidence. This is most visible in V@2 and V@10, where the CoDeR variants frequently outperform both dense retrievers and LLM-dependent baselines. The improvement supports the central design of CoDeR: topical relevance and constraint compatibility are related but separable signals, and combining them can produce a safer retrieved context for downstream RAG.

The results also reveal an inherent trade-off. A method that aggressively removes constraint-violating documents may lose some graded topical relevance, especially when the benchmark still assigns partial relevance to neutral topical documents. Therefore, a lower nDCG does not necessarily indicate a worse context for constraint-sensitive generation. In RAG settings where violating evidence can directly steer the generator toward an incorrect answer, reducing early violations can be more important than maximizing topical overlap alone.

Finally, the efficiency comparison separates CoDeR from LLM-dependent alternatives. Methods such as HyDE, NS-IR, and DEO can improve certain retrieval outcomes, but they require additional API calls and token consumption at inference time. CoDeR moves the constraint reasoning into a local encoder and therefore provides a cheaper and more private retrieval-side mechanism. The pending ablation study will further clarify how much of this behavior comes from the topical encoder, the compatibility encoder, and the integration policy.

